Neural Codec-based Adversarial Sample Detection for Speaker Verification

Automatic Speaker Verification (ASV), increasingly used in security-critical applications, faces vulnerabilities from rising adversarial attacks, with few effective defenses available. In this paper, we propose a neural codec-based adversarial sample detection method for ASV. The approach leverages the codec's ability to discard redundant perturbations and retain essential information. Specifically, we distinguish between genuine and adversarial samples by comparing ASV score differences between original and re-synthesized audio (by codec models). This comprehensive study explores all open-source neural codecs and their variant models for experiments. The Descript-audio-codec model stands out by delivering the highest detection rate among 15 neural codecs and surpassing seven prior state-of-the-art (SOTA) detection methods. Note that, our single-model method even outperforms a SOTA ensemble method by a large margin.

==> Figure_tex/codebook_layer_analysis.tex <==
\begin{figure}[t]
% \centering
\includegraphics[width=7.8cm]{Figures/Codebook_layer_analysis.png}
\caption{Codebook layer analysis using normalized edit distances (NED).}
\label{fig:ned_codebook_layers}
\end{figure}


==> Figure_tex/compare_with_scale_dr.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=8.0cm]{Figures/compare_with_scale_dr.png}
\caption{Comparing detection ratio with other methods under attack budgets $\epsilon=15$.} 
\label{fig:detection_ratio_epsilon10}
\end{figure}

==> Figure_tex/detection_rate_v.s._codecs.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=7.5cm]{Figures/detection_rate_v.s._codecs.png}
\caption{The detection ratio under attack budgets $\epsilon=10$.} 
\label{fig:detection_ratio_epsilon10}
\end{figure}


==> Figure_tex/kbps_codebook_num.tex <==
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.23\textwidth} % Adjust width as needed
        \centering
        \includegraphics[width=\textwidth]{Figures/kbps_genuine_eer.png}
        \caption{Bitrate vs Genuine EER}
        \label{fig:suba}
        \vspace{2mm} 
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.23\textwidth} % Adjust width as needed
        \centering
        \includegraphics[width=\textwidth]{Figures/kbps_adv_eer.png}
        \caption{Bitrate vs Adversarial EER}
        \label{fig:subb}
        \vspace{2mm} 
    \end{subfigure}
    \hfill
    % \begin{subfigure}[b]{0.22\textwidth} % Adjust width as needed
    %     \centering
    %     \includegraphics[width=\textwidth]{Figures/codebook_num_genuine_eer.png}
    %     \caption{CBN vs Genuine EER}
    %     \label{fig:subc}
    % \end{subfigure}
    % \hfill
    % \begin{subfigure}[b]{0.22\textwidth} % Adjust width as needed
    %     \centering
    %     \includegraphics[width=\textwidth]{Figures/codebook_num_adversarial_eer.png}
    %     \caption{CBN vs Adversarial EER}
    %     \label{fig:subd}
    % \end{subfigure}
    % \vspace{3mm}
    % \vspace{-2mm}
    \vspace{-4mm}
    \caption{Impact of bitrate on genuine and adversarial EER.}
    \label{fig:exp-kbps-codebook-num}
\end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.22\textwidth} % Adjust width as needed
%         \centering
%         \includegraphics[width=\textwidth]{Figures/kbps_genuine_eer.png}
%         \caption{Bitrate vs Genuine EER}
%         \label{fig:suba}
%         \vspace{2mm} 
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.22\textwidth} % Adjust width as needed
%         \centering
%         \includegraphics[width=\textwidth]{Figures/kbps_adv_eer.png}
%         \caption{Bitrate vs Adversarial EER}
%         \label{fig:subb}
%         \vspace{2mm} 
%     \end{subfigure}
%     \hfill
%     % \begin{subfigure}[b]{0.22\textwidth} % Adjust width as needed
%     %     \centering
%     %     \includegraphics[width=\textwidth]{Figures/codebook_num_genuine_eer.png}
%     %     \caption{CBN vs Genuine EER}
%     %     \label{fig:subc}
%     % \end{subfigure}
%     % \hfill
%     % \begin{subfigure}[b]{0.22\textwidth} % Adjust width as needed
%     %     \centering
%     %     \includegraphics[width=\textwidth]{Figures/codebook_num_adversarial_eer.png}
%     %     \caption{CBN vs Adversarial EER}
%     %     \label{fig:subd}
%     % \end{subfigure}
%     % \vspace{3mm}
%     \vspace{-2mm}
%     \caption{Exploring the impact of bitrate (kbps) and codebook number (CBN) on genuine and adversarial EER.}
%     \label{fig:exp-kbps-codebook-num}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.24\textwidth} % Adjust width as needed
%         \centering
%         \includegraphics[width=\textwidth]{Figures/kbps_genuine_eer.png}
%         \caption{Bitrate vs Genuine EER}
%         \label{fig:suba}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth} % Adjust width as needed
%         \centering
%         \includegraphics[width=\textwidth]{Figures/kbps_adv_eer.png}
%         \caption{Bitrate vs Adversarial EER}
%         \label{fig:subb}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth} % Adjust width as needed
%         \centering
%         \includegraphics[width=\textwidth]{Figures/codebook_num_genuine_eer.png}
%         \caption{CBN vs Genuine EER}
%         \label{fig:subc}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.24\textwidth} % Adjust width as needed
%         \centering
%         \includegraphics[width=\textwidth]{Figures/codebook_num_adversarial_eer.png}
%         \caption{CBN vs Adversarial EER}
%         \label{fig:subd}
%     \end{subfigure}
%     % \vspace{3mm}
%     \vspace{-2mm}
%     \caption{Exploring the impact of bitrate (kbps) and codebook number (CBN) on genuine and adversarial EER.}
%     \label{fig:exp-kbps-codebook-num}
% \end{figure}


==> Tables/compare_with_different_detect_methods.tex <==
\begin{table}[t]
\centering
\fontsize{8}{10}\selectfont
\setlength\tabcolsep{8pt}
\vspace{-3mm}
\caption{Compare detection rate with SOTA detection methods.}
\label{tab:diff_codec_fpr}
\vspace{-2mm}
\begin{tabularx}{0.4\textwidth}{c c c}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{2}{c}{Attack budget $\epsilon=15$} \\    
                  &  FPR =0.01  &  FPR = 0.001 \\
\midrule
 DAC D1           & \textbf{99.32} & \textbf{98.29} \\
 FunCodec F1      & 98.30 & 96.01  \\

Parallel WaveGAN  & 97.51 & 94.07  \\
HiFi-GAN          & 94.48 & 79.42  \\
Encodec           & 95.90 &  90.71 \\
Generation        & 97.62 & 94.71  \\
Gaussian          & 96.84 & 93.21  \\
Generation+Gaussian & 98.63 & 97.13  \\
 % None  & 95.65 & 90.57 & 74.05 &  2.88 \\
 % D1-Gau-0.05       &    &12.08&11.75&11.39 \\
 % D1-Gau-0.01       &    &8.64&7.11&5.85  \\
 % D1-Gau-0.01-FT       &    &    &  &5.37  \\
\bottomrule
\end{tabularx}
\end{table}


==> nouse/code_info.tex <==
\begin{table}[t]
\centering
\fontsize{8}{10}\selectfont
% \setlength\tabcolsep{5pt}
\caption{EER with different attack budgets $\epsilon$ using different Codecs. "A-F" represents different neural codec models, where "A" is SpeechTokenizer \cite{zhang2023speechtokenizer}, "B$\sim$" is AcademiCodec \cite{yang2023hifi}, "C" is AudioDec \cite{wu2023audiodec}, "D$\sim$" is DAC \cite{kumar2023high}, "E" is EnCodec \cite{defossez2022high}, and "F$\sim$" is FunCodec \cite{du2023funcodec}.}
% $n_c$ represents the codebook number, SR represents the sample rate, and BPS represents the bit rate in unit bits per second.
\label{tab:diff_codec_info}
\begin{tabularx}{0.43\textwidth}{lc c c c}
\toprule
% &  \multirow{2}{*}{Codec information} & \multicolumn{4}{c}{EER with different $\epsilon$ (\%)}           \\    
% &   & 15 & 10 & 5 & 0  \\
% &  \multirow{1}{*}{Codec information} & \multicolumn{4}{c}{EER with different $\epsilon$ (\%)}           \\    
&  Codec information & $N_q$ & BPS & SR  \\
% \midrule
%  & None  &  95.65  & 90.57   & 74.05  & 2.88  \\
\midrule
A    & 16k  &  8   &  4  &  16  \\
\midrule
B1 & hifi\_16k\_320d             &  4  &  2  &  16  \\
B2 & hifi\_16k\_320d\_large\_uni &  4  &  2  &  16  \\
B3 & hifi\_24k\_320d             &  4  &  3  &  24  \\
\midrule
C & 24k\_320d &  8  &  6.4  &  24  \\
\midrule
D1 & 16k &  12  &  6  & 16  \\
D2 & 24k &   32  &  24  & 24  \\
D3 & 44k &   9 &  8  & 44.1  \\
\midrule
E1 & 24k\_1.5bps &  2   & 1.5  & 24  \\
\midrule
F1 & en\_libritts\_16k\_gr1nq32ds320  &  32 & 16 & 16 \\
F2 & en\_libritts\_16k\_gr8nq32ds320  &  32 & 16 & 16 \\
F3 & en\_libritts\_16k\_nq32ds320     &  32 & 16 & 16 \\
F4 & en\_libritts\_16k\_nq32ds640     &  32 &  8 & 16 \\
% \cline{3-3}
F5 & zh\_en\_16k\_nq32ds320           &  32 & 16 & 16 \\
F6 & zh\_en\_16k\_nq32ds640           &  32 &  8 & 16 \\
\bottomrule
\end{tabularx}
\end{table}


==> nouse/detection_rate.tex <==
\begin{table}[t]
\centering
\fontsize{8}{10}\selectfont
\setlength\tabcolsep{4pt}
\caption{Detection rate with different attack budgets $\epsilon$.}
\label{tab:diff_codec_eer}
\vspace{-2mm}
\begin{tabularx}{0.42\textwidth}{c c c c c}
\toprule
\multirow{2}{*}{\small$FPR_{given}$} &  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Different $\epsilon$ (\%)} \\
&   & 15 & 10 & 5   \\
\midrule
\multirow{3}{*}{0.05} & DAC D1     & 99.72 &  99.02& 95.19  \\
                     & FunCodec F1      & 99.13& 98.08& 92.11  \\
                     & Parallel WaveGAN & 98.82&97.30&89.33 \\
\midrule
\multirow{3}{*}{0.01} & DAC D1   & 99.32 & 97.90 & 90.97 \\
     & FunCodec F1       & 98.30 & 96.32 & 86.31 \\
     & Parallel WaveGAN  & 97.56 & 94.76 & 81.60 \\
\midrule
\multirow{3}{*}{0.005} & DAC D1 & 99.09 & 97.42 & 89.00  \\
     & FunCodec F1       & 97.77 & 95.23 & 83.61  \\
     & Parallel WaveGAN  & 96.78 & 93.25 & 78.21  \\
\midrule
\multirow{3}{*}{0.001} & DAC D1  & 98.29 & 95.23 & 83.29 \\
     & FunCodec F1       & 96.01 & 92.39 & 76.40 \\
     & Parallel WaveGAN  & 93.89 & 88.60 & 68.58  \\
\bottomrule
\end{tabularx}
\end{table}


==> nouse/different_codec_eer.tex <==
\begin{table}[h]
\centering
\fontsize{8}{10}\selectfont
\setlength\tabcolsep{4pt}
\caption{EER with different attack budgets $\epsilon$ using different Codecs. "A-F" represents different neural codec models, where "A" is SpeechTokenizer \cite{zhang2023speechtokenizer}, "B$\sim$" is AcademiCodec \cite{yang2023hifi}, "C" is AudioDec \cite{wu2023audiodec}, "D$\sim$" is DAC \cite{kumar2023high}, "E" is EnCodec \cite{defossez2022high}, and "F$\sim$" is FunCodec \cite{du2023funcodec}.}
% $n_c$ represents the codebook number, SR represents the sample rate, and BPS represents the bit rate in unit bits per second.
\label{tab:diff_codec_eer}
\begin{tabularx}{0.49\textwidth}{lc c c c c}
\toprule
&  \multirow{2}{*}{Codec information} & \multicolumn{4}{c}{EER with different $\epsilon$ (\%)}           \\    
&   & 15 & 10 & 5 & 0  \\
\midrule
 & None  &  95.65  & 90.57   & 74.05  & 2.88  \\
\midrule
A    & 16k  &    & 17.31   &    &  4.62  \\
\midrule
B1 & hifi\_16k\_320d             &   & 15.44 &   & 6.21  \\
B2 & hifi\_16k\_320d\_large\_uni &   & 10.57 &   & 6.84  \\
B3 & hifi\_24k\_320d             &   & 22.00 &   & 6.62  \\
\midrule
C & 24k\_320d &   & 34.92 &    &  5.04  \\
\midrule
D1 & 16k & 40.75 & 29.31  &  15.84  & 3.32  \\
D2 & 24k &   & 30.67  &    & 3.00  \\
D3 & 44k &   &  29.65 &    & 3.44  \\
\midrule
% E1 & 24k\_1.5bps &   &   &   &   \\
% E2 & 24k\_3bps   &   &   &   &   \\
% E3 & 24k\_6bps   &   &   &   &   \\
% E4 & 24k\_12bps  &   &   &   &   \\
% E5 & 24k\_24bps  &   & 16.30  &   & 13.84  \\
E1 & 24k\_1.5kbps  &   & 16.30  &       & 13.84  \\
E2 & 24k\_6kbps    & 44.84 & 44.83  &  44.53 & 44.30  \\
E2 & 24k\_24kbps   & 44.71 & 44.27  & 43.97 & 43.82  \\
\midrule
F1 & en\_libritts\_16k\_gr1nq32ds320  & 66.16 & 50.97 & 27.93 & 3.45 \\
F2 & en\_libritts\_16k\_gr8nq32ds320  &       & 62.03 &       &  3.37  \\
F3 & en\_libritts\_16k\_nq32ds320     &       & 47.74 &       &  3.77 \\
F4 & en\_libritts\_16k\_nq32ds640     &       & 36.27 &       &  4.05 \\
% \cline{3-3}
F5 & zh\_en\_16k\_nq32ds320           &       & 47.37 &    & 3.51  \\
F6 & zh\_en\_16k\_nq32ds640           &       & 38.64 &    & 3.37  \\
\bottomrule
\end{tabularx}
\end{table}


==> nouse/different_speaker_eer.tex <==
\begin{table}[t]
\centering
\fontsize{8}{10}\selectfont
\caption{EER with different attack budgets $\epsilon$.}
\label{tab:diff_codec_eer}
\vspace{-2mm}
\begin{tabularx}{0.4\textwidth}{c c c c c}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{3}{c}{Different $\epsilon$ (\%)} \\    
                  &  15  &  10  &  5  &  0  \\
\midrule
 DAC D1           & 40.75 & 29.31 & 15.84 &  3.32 \\
 FunCodec F1      & 66.16 & 50.97 & 27.93 &  3.45 \\
 Parallel WaveGAN  & 65.75 & 52.20 & 30.37 &  3.39 \\
 None  & 95.65 & 90.57 & 74.05 &  2.88 \\
\bottomrule
\end{tabularx}
\end{table}


==> nouse/nouse_discrete_unit_comparison.tex <==
\begin{table}[t]
\centering
\fontsize{8}{10}\selectfont
\setlength\tabcolsep{10pt}
\caption{The edit distance of discrete unit}
% $n_c$ represents the codebook number, SR represents the sample rate, and BPS represents the bit rate in unit bits per second.
\label{tab:diff_codec_eer}
\begin{tabularx}{0.47\textwidth}{l c c c c}
\toprule
  \multirow{2}{*}{Method} & \multicolumn{4}{c}{EER with different $\epsilon$ (\%)} \\    
&    20  & 15 & 10 & 5   \\
\midrule
 % None  &  11.11  & 11.11   & 11.11 & 11.11 \\
 D1       &    &    & 98532  &  \\
 F1       &    &    &  &  \\
 D1-Gau-0.05       &    &    &  &  \\
 D1-Gau-0.01       &    &    &  &  \\
 D1-Gau-0.01-FT       &    &    &  41437  &  \\
\bottomrule
\end{tabularx}
\end{table}

